MotorEase: Automated Detection of Motor Impairment Accessibility Issues in Mobile App UIs

Recent research has begun to examine the potential of automatically finding and fixing accessibility issues that manifest in software. However, while recent work makes important progress, it has generally been skewed toward identifying issues that affect users with certain disabilities, such as those with visual or hearing impairments. However, there are other groups of users with different types of disabilities that also need software tooling support to improve their experience. As such, this paper aims to automatically identify accessibility issues that affect users with motor-impairments. To move toward this goal, this paper introduces a novel approach, called MotorEase, capable of identifying accessibility issues in mobile app UIs that impact motor-impaired users. Motor-impaired users often have limited ability to interact with touch-based devices, and instead may make use of a switch or other assistive mechanism -- hence UIs must be designed to support both limited touch gestures and the use of assistive devices. MotorEase adapts computer vision and text processing techniques to enable a semantic understanding of app UI screens, enabling the detection of violations related to four popular, previously unexplored UI design guidelines that support motor-impaired users, including: (i) visual touch target size, (ii) expanding sections, (iii) persisting elements, and (iv) adjacent icon visual distance. We evaluate MotorEase on a newly derived benchmark, called MotorCheck, that contains 555 manually annotated examples of violations to the above accessibility guidelines, across 1599 screens collected from 70 applications via a mobile app testing tool. Our experiments illustrate that MotorEase is able to identify violations with an average accuracy of ~90%, and a false positive rate of less than 9%, outperforming baseline techniques.

==> macro.tex <==

\usepackage{ifthen}

\makeatletter

% this  is a easy way to add and highlight new text  ...
% just comment in/out the \tnew macro ..

\newcommand{\tnew}[1]{{\bf { #1 }} }
%\newcommand{\tnew}[1]{{ { #1 }} }

% math and theorem definition

\newcommand{\ndef}{\stackrel{\rm def}{=}}

% this is used for draft only

%\renewcommand{\baselinestretch}{2}

% just to number pages in the draft

\pagenumbering{arabic}

% nothing i.e., no-numbering final and camera ready

%\pagestyle{empty}


\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\ie}{\textit{i.e.},\xspace}
\newcommand{\eg}{\textit{e.g.},\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\aka}{\textit{a.k.a.}\xspace}


\definecolor{mycolor}{RGB}{204,204,204}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\small{\textbf{
			\node[shape=circle,fill=mycolor,draw=black, inner sep=0.75pt] (char) {\textcolor{black}{#1}};}}}}

\newcommand*\circld[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=0.5pt] (char) {#1};}}

\newboolean{showcomments}


\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\cvsversion}{\emph{\scriptsize$-$Id: macro.tex,v 1.9 2005/12/09 22:38:33 giulio Exp $}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\cvsversion}{}
  }

%% Merge citations into single brackets with commas
%\usepackage[noadjust]{cite}
%\renewcommand{\citepunct}{,\penalty\citepunctpenalty\,}
%\renewcommand{\citedash}{--}% optionally


\newcommand{\REF}{{\color{red} \textbf{[REFS]}}\xspace}
\newcommand\oscar[1]{\textcolor{olive}{\nb{OSCAR}{#1}}}
\newcommand\NATHAN[1]{\textcolor{blue}{\nb{NATHAN}{#1}}}
\newcommand\DENYS[1]{\textcolor{violet}{\nb{DENYS}{#1}}}
\newcommand\CARLOS[1]{\textcolor{orange}{\nb{CARLOS}{#1}}}
\newcommand\KEVIN[1]{\textcolor{violet}{\nb{KEVIN}{#1}}}
\newcommand{\num}{{\color{red} \textbf{XX}}\xspace}

\newcommand\revision[1]{{{#1}}}



\newcommand{\tango}{{\sc Tango}\xspace}
\newcommand{\tangolong}{{\sc de\textbf{T}ecting duplic\textbf{A}te scree\textbf{N} recordin\textbf{G}s of s\textbf{O}ftware bugs}\xspace}


\newcommand{\tangot}{{\sc Tango$_{txt}$}\xspace}
\newcommand{\tangov}{{\sc Tango$_{vis}$}\xspace}
\newcommand{\tangoc}{{\sc Tango$_{comb}$}\xspace}


\newcommand{\bflcs}{B+f-LCS\xspace}
\newcommand{\bwlcs}{B+w-LCS\xspace}

==> texs/6_limitations.tex <==
\section{Threats to Validity}
\label{sec:limits}
%LIMITATIONS

%- where does MotorEase lack 

%- it does not overlook all guidelines and only looks at a handful 

%MIRCALE's results are encouraging and optimistic as a tool that is able to detect motor-impaired accessibility issues within an application. MotorEase, however, is not without its limitations. This section will take a look at situations in which MotorEase is limited the validity of the tool and its detectors. 

%MotorEase's dependency on the availability of dynamically produced XML information makes it less accurate when XML information is not correctly represented. Software developers tend to not label their elements in applications \cite{Chen20}, therefore making if difficult for MotorEase to properly identify elements on the screen. 

%MIRCALE is unable to detect violations with the same level of accuracy and precision in apps that are not open source. Popular applications wish accessibility violations may not be detected since MotorEase does not have access to the source code in order to generate the dynamic screenshot and XML elements. 
\revision{

\noindent\textbf{Internal Validity:} The main threat to the internal validity of our study is the construction of the \MotorCheck benchmark. However, we mitigated this threat by constructing the dataset with input from two authors, who mutually agreed on the selected violation sets.

\noindent\textbf{Construct Validity:} The main threat to the construct validity of our experiments is related to the measurement of our approach compared to the ground truth. However, two authors manually verified \MotorEase's output as compared to the ground-truth.

\noindent\textbf{External Validity:} Threats to external validity of our study are mainly concerned with the generalizability of our approach and dataset. The dataset used to test \MotorEase was a compilation of screenshots and \texttt{\small XML} files from a large number of popular apps. However, we cannot claim that our current results generalize beyond the dataset used. However, this threat to external validity is mitigated due to the size, diversity, and popularity of the apps used. 


}



































